Cross-Lingual Transfer Learning for Statistical Type Inference

Hitherto statistical type inference systems rely thoroughly on supervised learning approaches, which require laborious manual effort to collect and label large amounts of data. Most Turing-complete imperative languages share similar control- and data-flow structures, which make it possible to transfer knowledge learned from one language to another. In this paper, we propose a cross-lingual transfer learning framework, PLATO, for statistical type inference, which allows us to leverage prior knowledge learned from the labeled dataset of one language and transfer it to the others, e.g., Python to JavaScript, Java to JavaScript, etc. PLATO is powered by a novel kernelized attention mechanism to constrain the attention scope of the backbone Transformer model such that the model is forced to base its prediction on commonly shared features among languages. In addition, we propose the syntax enhancement that augments the learning on the feature overlap among language domains. Furthermore, PLATO can also be used to improve the performance of the conventional supervised learning-based type inference by introducing cross-lingual augmentation, which enables the model to learn more general features across multiple languages. We evaluated PLATO under two settings: 1) under the cross-domain scenario that the target language data is not labeled or labeled partially, the results show that PLATO outperforms the state-of-the-art domain transfer techniques by a large margin, e.g., it improves the Python to TypeScript baseline by +5.40%@EM, +5.40%@weighted-F1, and 2) under the conventional monolingual supervised learning based scenario, PLATO improves the Python baseline by +4.40%@EM, +3.20%@EM (parametric).

==> tex/background.tex <==
\section{Background}\label{sec:back}

In this section, we introduce the fundamentals of statistical type inference, attention mechanism and masked language modeling.

\subsection{Statistical Type Inference}
Statistical type inference adopts statistical model for the prediction of variables, parameters and
function return
types. Concisely, statistical model predicts the types of tokens in a code sequence using the
contextual information
(\ie, all the other tokens in the input sequence) within. Currently, these models are learned in a
supervised manner via
gradient-based training process on manually labelled dataset which requires substantial human effort and domain
knowledge.
% \yi{Need to talk about traditional supervised learning-based type inference: code sequences,
% training, prediction, etc.}

\subsection{Attention Mechanism}
% Proposed by Vaswani et al., the traditional dot-product (multiplicative) attention aggregation mechanism is as:

% \begin{equation}
% \mathrm{P}(v_{q}|q,\mathrm{K}) = attn_{k, v}(q) = \sum_{k\in \mathrm{K}}\alpha_{q,k}v_k =
%\sum_{k\in \mathrm{K}} \frac{qk}{\mathrm{Z}}v_k
% \label{vanattn}
% \end{equation}

Given a word sequence, attention mechanism~\cite{vaswani2017attention} tries to calculate word
embedding for each of the words in the sequence.
Basically, an embedding of a word (\emph{center word}) is the weighted average of the embeddings of
all the other words (\emph{context words}) in the sequence, and the weights, known as the
attention, are measured by the relation of the \emph{center word} with all the \emph{context words} in the sequence.
The detailed formula is as follows:%
{\small\begin{equation}
\mathbf{attention(q,\mathrm{K}) = \sum_{k\in \mathrm{K}}\alpha_{q,k}k = \sum_{k\in \mathrm{K}}
\frac{\langle q,k \rangle}{\mathrm{Z}}k}.
\label{vanattn}
\end{equation}}
\looseness=-1
Specifically, given a \emph{center word} embedding $\mathbf{q\in \mathbb{R}^{d_{model}}}$ ($\mathbb{R}^{d_{model}}$ is the dimension of the latent representation used in a model), attention computes its cosine similarity with all the \emph{context word} embeddings $\mathbf{k\in \mathbb{R}^{d_{model}}}$ within the sequence, which gives the attention weights $\mathbf{\alpha_{q,k}}$. Finally the aggregated representation of $\mathbf{q}$ is calculated as the average of $\mathbf{k}$ weighted by $\mathbf{\alpha_{q,k}}$. Noted that $\mathbf{Z}$ is a normalization term.


\subsection{Self-Supervised Pre-Training}\label{mlm}
Previous work~\cite{devlin2018bert,brown2020language,jesse2021learning} observed that instead of
directly training a model with a supervised task-specific loss, model often benefit from combining
with a self-supervised pre-training stage. Popular pre-training objectives include: \emph{masked language modeling} (MLM), \emph{next sentence prediction} (NSP), etc. Specifically, given an input sequence, MLM masks a certain proportion of tokens within, and let the model predict the words at the masked positions based on the other context words in the input
sequence. The formula of MLM loss is as follows:
\vspace{-5pt}\noindent\par{\small\begin{equation}
\mathcal{L}_{\mathrm{MLM} } = \mathbf{\sum_{\mathrm{x_{[MASK]}}\in \mathrm{\mathbf{x} _{[MASK]} }}  \mathrm{-log(P(x_{[MASK]}|\mathbf{x} \backslash x_{[MASK]}))}}
\end{equation}}
where $\mathbf{x}$ is the input sequence and $\mathrm{\mathbf{x} _{[MASK]} }$ is the set of tokens that are masked. For NSP, it trains the model to embed the sequence-level knowledge by forcing it to classify whether one sequence follows another. Inspired by the boost one can gain from pretraining, XLM~\cite{lample2019cross} introduces a cross-language
model by training BERT~\cite{devlin2018bert} (an attention based model) language model with corpus
from multiple natural language sources and is shown to improve performance on cross-lingual tasks.
In this paper, we train a language model with dataset from different programming language sources as
the backbone model, which is referred to as a \emph{cross-programming-language model} (XPLM).


% \subsection{limitations of traditional attention}
% % introduce limitation of traditional attention on program analysis task
% As our proposed method is based on BERT \cite{devlin2018bert}, here we discuss the limitation of the attention module of BERT when applying it to programming analysis task.

% In traditional attention, the embedding of a word depends on its relations with all the other
%words in an input sequence, \ie there is no constraint to its attention scope. For example,
%consider a code sequence $var~a = true;~ var~b = 0$, when calculating embedding for token $a$, the
%traditional attention mechanism considers its relations with all the other tokens in the input
%sequence. However, it is apparent that $var~b = 0;$ is totally irrelevant to the type information
%of $a$, thus it is possible that model would erroneously base its prediction on $b$ or $0$ which
%is
%devastating for prediction and generalization.

==> tex/future.tex <==
\section{Future work}
In this work, we have demonstrated the effectiveness of our method on the attention-based BERT architecture. Our framework is general and in the future we plan to incorporate it into other model architectures such as bidirectional recurrence neural networks or graph neural networks to further improve their performance. Anthoer interesting direction is to adapt our framework to other neural-based software engineering tasks such as code summarization or bug detection.
